SEvenLLM: Benchmarking, Eliciting, and Enhancing Abilities of Large Language Models in Cyber Threat Intelligence

To address the increasing complexity and frequency of cybersecurity incidents emphasized by the recent cybersecurity threat reports with over 10 billion instances, cyber threat intelligence (CTI) plays a critical role in the modern cybersecurity landscape by offering the insights required to understand and combat the constantly evolving nature of cyber threats. Inspired by the powerful capability of large language models (LLMs) in handling complex tasks, in this paper, we introduce a framework to benchmark, elicit, and improve cybersecurity incident analysis and response abilities in LLMs for Security Events (SEvenLLM). Specifically, we create a high-quality bilingual instruction corpus by crawling cybersecurity raw text from cybersecurity websites to overcome the lack of effective data for information extraction. Then, we design a pipeline to auto-select tasks from the tasks pool and convert the raw text into supervised corpora comprised of question and response. The instruction dataset SEvenLLM-Instruct is used to train cybersecurity LLMs with the multi-task learning objective (27 well-designed tasks) for augmenting the analysis of cybersecurity events. Extensive experiments in our curated benchmark (SEvenLLM-bench) demonstrate that SEvenLLM performs more sophisticated threat analysis and fortifies defenses against the evolving landscape of cyber threats.

==> evaluation-result.tex <==
\subsection{Evaluation}
\paragraph{GPT-4 Score} To score the standard answers of the test set and the answers provided by the trained model, we set the evaluation criteria as \{very pool: 1, slightly poor: 2, neutral: 3, good: 4, very good: 5\} to compute the score. 

\paragraph{Rouge-L Score} We use Rouge-L to evaluate the output of the LLM, which is tokenized by space in English and jieba\footnote{\url{https://github.com/fxsjy/jieba}} in Chinese.


\paragraph{Semantic Score} Using the multilingual sentence-transformers model\footnote{\url{https://huggingface.co/sentence-transformers/paraphrase-multilingual-MiniLM-L12-v2}} \cite{reimers-sentence-bert}, we map the text to a 384-dimensional dense vector space. This can be used for tasks such as clustering or semantic search, allowing for the evaluation of whether the values in a test dictionary can score from a semantic understanding perspective. This approach is more aligned with the open-ended nature of cyber security event analysis. Due to its support for various lengths and both Chinese and English languages, this model is applied to both understanding and generation tasks. 

\paragraph{Multiple-choice Question Score} we designed 100 multiple-choice questions for two languages and two major types of tasks to comprehensively evaluate the model's capabilities. The output results were manually verified to ensure an effective assessment of the model's ability to handle objective questions.

\section{Main Results}
\paragraph{GPT-4 Evaluation} 
In Table \ref{tab:gpt4score}, compared to the results of models that have not been trained with \instruct{}, it is evident that training with the datasets provided in this work significantly improves performance. Additionally, it is observed that while higher-capacity models show improvements in multiple-choice questions, they can occasionally perform worse in fuzzy testing and semantic similarity matching. This reinforces the previous analysis and highlights that within the sub-20B parameter range, larger models may not necessarily include more content in the domain of cybersecurity event analysis within their pre-training corpora. Considering that cybersecurity data is challenging to collect and highly specialized, this underscores the importance of enhancing training materials in this field with datasets like those provided in this paper. It has also been observed that base models can perform correct analysis but still produce incorrect answers, indicating that the full potential of an AI model requires not only general training but also alignment with specialized corpora to yield more accurate outcomes.


\paragraph{Rouge-L\&Semantic Evaluation} In Table \ref{tab:rougelscore} and Table \ref{tab:semanticscore}, numerous repetitive outputs are observed in Qwen-14B-Chat, which is a tendency in language model decoding to increase the probability of repeating previous sentences. Since the parameters are consistent with the 7B model, it is inferred that higher parameter models may require adjustments to the repetition\_penalty and temperature settings. Furthermore, using Llama-2-13b with CoT, where the model is guided to reason before outputting a result, did not outperform the non-CoT-aided 13B model either in fuzzy matching or similarity matching, and only performed comparably in multiple-choice questions without constructing CoT. This supports the analysis that within the 7B-13B parameter range, the introduction of guided thinking may lead to more rigid model behavior and does not necessarily improve performance. 


\paragraph{Multiple-choice Question} In Table \ref{tab:mcqscore}, during a comparison of multiple-choice questions, it is observed that the Qwen performs less effectively than Llama2, particularly in scenarios requiring a degree of reasoning and where answers may be confusing. This includes questions where certain options included content from the original text, where Qwen had trouble identifying correctly. The LLMs with 13B and 14B parameters have been confirmed to perform better in multiple-choice question scenarios. However, there have been mixed results in terms of semantic similarity and fuzzy matching. This suggests that the enrichment of overall knowledge and reasoning capabilities with larger model sizes improves performance in multiple-choice questions, but the increased volume of information can lead to more divergent responses, which may not always align well with strict fuzzy and semantic matching tests in the test set. To corroborate this, the results of Llama-2-13B were scored using GPT-4, which showed an improvement, indicating that a larger model size results in richer descriptions, supporting the analysis.


